Robust Cross-lingual Hypernymy Detection using Dependency Context

Cross-lingual Hypernymy Detection involves determining if a word in one language ("fruit") is a hypernym of a word in another language ("pomme" i.e. apple in French). The ability to detect hypernymy cross-lingually can aid in solving cross-lingual versions of tasks such as textual entailment and event coreference. We propose BISPARSE-DEP, a family of unsupervised approaches for cross-lingual hypernymy detection, which learns sparse, bilingual word embeddings based on dependency contexts. We show that BISPARSE-DEP can significantly improve performance on this task, compared to approaches based only on lexical context. Our approach is also robust, showing promise for low-resource settings: our dependency-based embeddings can be learned using a parser trained on related languages, with negligible loss in performance. We also crowd-source a challenging dataset for this task on four languages -- Russian, French, Arabic, and Chinese. Our embeddings and datasets are publicly available.

==> models.tex <==
\ignore{
As discussed earlier, a unsupervised approach for detecting lexical entailment requires a) {\em feature representations} for the words and b) a {\em scoring function} (preferably asymmetric) that measures the strength of the entailment relationship. We follow the setup proposed by \newcite{Vyas2016} for detecting lexical entailment cross-lingually, which we describe below.
}
% We describe each of the two components as used in their framework separately. First, we describe their novel model for obtaining sparse, bilingual representations. Second, we describe \balapinc, the scoring function that aims to capture entailment using the proposed representations.

\ignore{
\subsection{Sparse, Bilingual Word Representations for Cross-lingual Entailment}
To generate feature representations for words in both languages jointly, \newcite{Vyas2016} propose \textsc{BiSparse} - a model to obtain sparse, bilingual word representations. \textsc{BiSparse} is based on non-negative matrix factorization with sparsity inducing $l_1$ penalty. Specifically, they start with monolingual embeddings for the two languages  $\mathbf{X_e}$ and $\mathbf{X_f}$, of sizes  $v_e \times n_e$ and $v_f \times n_f$ respectively. Next, they define a ``score'' matrix $\mathbf{S}$ of size $v_e \times v_f$, which captures correspondences between the vocabularies of the two languages. Each row of $\mathbf{S}$ is a one-hot vector that identifies the word in \textbf{\emph{f}} that is most frequently aligned with the \textbf{\emph{e}} word for that row in a large parallel corpus. To obtain the final sparse, bilingual embeddings, the following optimization problem is solved :

	\begin{align*}
	\label{eqn:bisparse}
	\underset{\mathbf{A_e, D_e, A_f, D_f} }{\text{argmin~}}& \sum\limits_{i=i}^{v_e}  \; \frac{1}{2}|| \mathbf{A_e}_{i}\mathbf{D_e}^{\text{T}} - \mathbf{X_e}_i  ||^2_2 \; + \lambda_e||\mathbf{A_e}_i||_1 \;\\                                
	+& \sum\limits_{j=i}^{v_f}  \; \frac{1}{2}|| \mathbf{A_f}_j\mathbf{D_f}^{\text{T}} - \mathbf{X_f}_j ||^2_2 \; + \lambda_f||\mathbf{A_f}_j||_1 \; \\          
	+& \sum\limits_{i=1}^{v_e} \sum\limits_{j=1}^{v_f}  \frac{1}{2} \lambda_x \mathbf{S}	_{ij} || \mathbf{A_e}_i - \mathbf{A_f}_j ||_2^2 \numberthis\\  
	{\text{subject to ~} }    &\mathbf{A_{e}} > 0\; ; {\mathbf{D_e}_i}^{\text{T}}.\mathbf{D_e}_i \leq 1, 1 \leq i \leq v_e ;\\
	&\mathbf{A_{f}} > 0\;  ; {\mathbf{D_f}_j}^{\text{T}}.\mathbf{D_f}_j \leq 1, 1 \leq j \leq v_f ;\\
	\end{align*}
The first two rows and the constraints in Equation \ref{eqn:bisparse} encourage sparsity and non-negativity in the final word representations for each language. The third row imposes bilingual correspondence constraints, weighted by the regularizer $\lambda_x$: it encourages words in \textbf{\emph{e}} and \textbf{\emph{f}} that are strongly aligned according to  $\mathbf{S}$ to have similar representations.

An attractive property of this setup is that it allows us to examine the effectiveness of different contexts seamlessly, by simply choosing appropriate $\mathbf{X_e}$ and $\mathbf{X_f}$. For instance, \newcite{Vyas2016} use GloVe vectors \cite{Pennington2014} as their $\mathbf{X_e}$ and $\mathbf{X_f}$, which is equivalent to using embeddings with window context (we call this model \textsc{BiSparse-Lex}). In this work, we use the different dependency based contexts described in Section \ref{sec:depend-based-word} to induce $\mathbf{X_e}$ and $\mathbf{X_f}$, and we collectively call these models \textsc{BiSparse-Dep}.\yv{Needs more emphasis as this is key difference}

\subsection{Determining Entailment}
Detecting lexical entailment without supervision requires a scoring function which quantifies the \emph{directional} semantic similarity of an input word pair. Again, we follow \newcite{Vyas2016} and use use the \balapinc score \cite{kotlerman2009directional}, which is based on the distributional inclusion hypothesis \cite{Geffet2005}: given feature representations of the contexts of two words $u$ and $v$,  $u$ is assumed to entail $v$ if all features of $u$ tend to appear within the features of $v$. 

Formally, \balapinc is the geometric mean of a symmetric similarity score, \emph{LIN}  \cite{lin1998automatic}, and an asymmetric score, \emph{APinc}. Given a directional entailment pair ($u$ $\rightarrow$ $v$),
\begin{align*}
\text{\emph{balAPinc}}(u \rightarrow v) = \sqrt{\text{\emph{LIN}}(u,v)\cdot\text{\emph{APinc}}(u \rightarrow v)}
\end{align*}

\ignore{Assume we are given ranked feature lists $FV_u$ and $FV_v$ for words $u$ and $v$ respectively. Let $w_u(f)$ denote the weight of a particular feature $f$ in $FV_u$.  \emph{LIN} is defined by 

\vspace{-0.25in}
\begin{align}
\text{\emph{LIN}}(u,v) = \frac{\sum\limits_{f \in FV_u \cap FV_v} [w_u(f) + w_v(f)]}{\sum\limits_{f \in FV_u} w_u(f) + \sum\limits_{f \in FV_v} w_v(f)}
\end{align}

\emph{APinc} is a modified asymmetric version of the Average Precision metric used in Information Retrieval:

\vspace{-0.25in}
\begin{align}
\text{\emph{APinc}}(u \rightarrow v) = \frac{\sum\limits_{r = 1}^{\vert FV_u \rvert}[P(r,FV_u,FV_v)\cdot rel'(f_r)]}{\lvert FV_u \rvert}
\end{align}
\vspace{-0.1in}
where, \begin{align*}
&P(r,FV_u,FV_v) \\
&~~~~~~~~~~~= \frac{\text{\# of features of \emph{v} in top \emph{r} features of \emph{u} }}{r} \\
&rel'(f,FV_v) = \begin{cases}
1 - \frac{rank(f,FV_u)}{\lvert FV_u \rvert + 1} & \text{if} f \in FV_u \\	
0 & \text{otherwise}\\
\end{cases}
\end{align*}
}

\balapinc has two tunable parameters - a threshold $t$ that indicates the \balapinc score above which all examples are labeled as positive, and $K$, the maximum number of features to consider for each word.
}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% TeX-PDF-mode: t
%%% End: 


==> prelim.tex <==
% \yv{This seems out of place here}
% Indeed, hypernymy is one of the predominant relationship in existing
% monolingual entailment datasets\cite{Baroni2011,??}.

% \mc{There is a lot of background before getting to the contributions. At the same time, the paper has no "Related Work" section.}

% \subsection{Cross-Lingual Entailment}



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% TeX-PDF-mode: t
%%% End: 


==> qual.tex <==
\paragraph{Qualitative Analysis}
We qualitatively analyze the differences between the window and the
dependency based models by comparing the predictions of
\textsc{BiSparse-Dep} (Full) and \textsc{BiSparse-Lex} (Table \ref{tab:qual}).

The window model has difficulty capturing functional relations, such
as {\em époux} (spouse in French) is a {\em relative} or
{\em \foreignlanguage{russian}{бас}} (bass in Russian) is an
{\em instrument}. For false positives, the window model often ignores the
directional nature, predicting {\em vêtement} (clothing in French) is a {\em jeans} or
{\em \foreignlanguage{russian}{ткань}} (Russian for tissue) 
is a
{\em nerve} as positive instances. In contrast, the \textsc{BiSparse-Dep}
can capture the functional similarity and directionality correctly for
all these instances.

\begin{table}
  \footnotesize
  \centering
  \begin{tabular}{l|l}
  False Negatives & False Positives \\
  \toprule
  (pêcheur (en:fisher), worker) &  (vêtement (en:clothing), jeans) \\ % campaign/countryside, race and clothing, jeans
  (époux (en:spouse), relative) & (cercueil (en:coffin), casket) \\ % spouse, relative and coffin, casket
  (équipe (en:team), unit) & (statut (en:status), barony) \\ % team, unit and 
  \midrule 
  % (\foreignlanguage{russian}{бас} (en:bass), instrument) & (\foreignlanguage{russian}{художник} (en:artist), illustrator) \\ % bass/bass, instrument and artist, illustrator
  (\foreignlanguage{russian}{бас} (en:bass), instrument) & (\foreignlanguage{russian}{ткань} (en:tissue), nerve) \\
  (\foreignlanguage{russian}{замок} (en:castle), structure) & (\foreignlanguage{russian}{флора} (en:flora), sunflower) \\ % castle/lock, structure and flora, sunflower
  (\foreignlanguage{russian}{трейлер} (en:trailer), vehicle) & (\foreignlanguage{russian}{чувство} (en:feeling), cynicism) \\ % trailer/trailer, vehicle and feeling, cynicism
  % (buveur,consumer) & (oiseau,parrot) \\
  % (aristocratie,class) & (criminel,smuggler)\\
  % (\foreignlanguage{russian}{надежда}, feeling) & (\foreignlanguage{russian}{здание}, observatory) \\
  % (\foreignlanguage{russian}{нефть}, substance) & (\foreignlanguage{russian}{симптом}, edema) \\
  \bottomrule
\end{tabular}
\caption{Errors made by the \textsc{BiSparse-Lex} model. Our \textsc{BiSparse-Dep} model predicted them correctly. See text for details.}
\label{tab:qual}
\end{table}

Many test pairs
were hard due to translation ambiguity. \todo{decide to add more if space permits}
% For instance, in ({\em dessous},{\em garment}) from the French
% dataset, {\em dessous} can be translated to {\em underneath},
% however the apt translation is {\em underwear} in this example.  For
% another French pair ({\em poire},{\em fruit}), the word {\em poire}
% can be translated to {\em perry}, which is a drink, but the apt
% translation is {\em pear}.  Similarly, for the Russian pair
% (\foreignlanguage{russian}{лук}, {\em produce}),
% \foreignlanguage{russian}{лук} can be translated to {\em bow}, but
% the apt translation is {\em onion}.  In
% (\foreignlanguage{russian}{глава}, leader),
% \foreignlanguage{russian}{глава} can be incorrectly translated to
% {\em chapter}, but the apt translation is {\em head}.

% frappeur player

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% TeX-PDF-mode: t
%%% End: 

